A Survey of Predictive Maintenance: Systems, Purposes and Approaches

This paper highlights the importance of maintenance techniques in the coming industrial revolution, reviews the evolution of maintenance techniques, and presents a comprehensive literature review on the latest advancement of maintenance techniques, i.e., Predictive Maintenance (PdM), with emphasis on system architectures, optimization objectives, and optimization methods. In industry, any outages and unplanned downtime of machines or systems would degrade or interrupt a company's core business, potentially resulting in significant penalties and immeasurable reputation and economic loss. Existing traditional maintenance approaches, such as Reactive Maintenance (RM) and Preventive Maintenance (PM), suffer from high prevent and repair costs, inadequate or inaccurate mathematical degradation processes, and manual feature extraction. The incoming fourth industrial revolution is also demanding for a new maintenance paradigm to reduce the maintenance cost and downtime, and increase system availability and reliability. Predictive Maintenance (PdM) is envisioned the solution. In this survey, we first provide a high-level view of the PdM system architectures including PdM 4.0, Open System Architecture for Condition Based Monitoring (OSA-CBM), and cloud-enhanced PdM system. Then, we review the specific optimization objectives, which mainly comprise cost minimization, availability/reliability maximization, and multi-objective optimization. Furthermore, we present the optimization methods to achieve the aforementioned objectives, which include traditional Machine Learning (ML) based and Deep Learning (DL) based approaches. Finally, we highlight the future research directions that are critical to promote the application of DL techniques in the context of PdM.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> ack.tex <==
\section*{Acknowledgment}
This work is supported in part by .


==> knowledge.tex <==
\section{Knowledge Based Approaches}
\label{knowledge}


%Diagnosis is the ability to detect fault, isolate and identify which component is failure, and decide on the potential impact of failed component on the health of the system. Fault detection is a task to indicate whether something is going wrong in the monitored system; fault isolation is a task to locate the component that is faulty; and fault identification is a task to determine the nature of the fault when it is detected.

%Prognosis is the capability to use available observations to predict upcoming states of machine or forecast the fault before it occurs. 
%Fault detection is a task to indicate whether something is going wrong in the monitored system; fault isolation is a task to locate the component that is faulty; and fault identification is a task to determine the nature of the fault when it is detected. 
%The literature on diagnosis and prognosis is huge and diverse primarily due to a wide variety of systems, components and parts. In this section, we mainly investigate the approaches for fault diagnosis and prognosis disregarding the types of systems or components to provide the information for research’s community.
%The approaches for diagnosis and prognosis in a PdM system can be classified into two basic categories: knowledge-based and data-driven approaches. A detailed taxonomy of PdM approaches is illustrated in Fig. \ref{fig:approaches}.
%\begin{figure}[htbp]
%\centering
%\includegraphics[width=3.5in]{./fig/approaches.eps}
%\caption{Taxonomy of PdM approaches.}
%\label{fig:approaches}
%\end{figure}

Most traditional PdM methods for fault diagnosis and prognosis depend on a priori expert knowledge and deductive reasoning process, e.g. expert systems and model-based reasoning. In this section, we briefly review the knowledge-based approaches applied in diverse systems, with a complete list of references. Typically, we classify the knowledge-based approaches into three categories: ontology-based, rule-based and model-based approaches.

\subsection{Ontology-based Approaches}
An ontology formally describes the context knowledge through concepts and relationships that exist in a particular area of concentration or specific domain. A general procedure of an ontology construction \cite{konys2018ontology} is illustrated in Fig. \ref{fig:ontology}. Ontology-based context modeling allows \cite{wang2004ontology}: knowledge sharing between computational entities by having a common set of concepts, logic inference by exploiting various existing logic reasoning mechanisms to deduce high-level, conceptual context from low-level and raw context, and knowledge reuse by reusing well-defined ontologies of different domains. 

%consists of the following phases: (1) defining a set of criteria; (2) taxonomy construction; (3) ontology construction; (4) formal description; (5) defined classes creation; (6) reasoning process; (7) consistency verification; and (8) a set of results. 

\begin{figure*}[htbp]
\centering
\includegraphics[width=7in]{./fig/ontology.eps}
\caption{A general procedure of an ontology construction (adapted from \cite{konys2018ontology}).}
\label{fig:ontology}
\end{figure*}

Ontology can be employed to establish knowledge base for diverse machinery systems and devices, and can be combined with various existing reasoning algorithms (e.g., rule-based reasoning, Kalman filter, and ANN) to achieve fault diagnosis and prognosis. Different ontologies have been constructed for PdM or health assessment systems \cite{konys2018ontology, schmidt2017semantic, nunez2018ontoprog}. For example, Konys \cite{konys2018ontology} propose a structured and ontology-based knowledge model for sustainability assessment domain. Schmidt \emph{et al.} \cite{schmidt2017semantic} develop a semantic framework, using an ontology-based approach for data aggregation, to support context-aware and cloud-enabled maintenance of manufacturing assets. Medina-Oliva and Voisin \emph{et al.} \cite{medina2014predictive, voisin2013fleet} present a fleet-wide approach based on ontologies in order to capitalize on knowledge and applied relevant vector machine to achieve predictive diagnostic in the marine domain. Reasoning over ontology is powerful to capture and formalize the context information of PdM systems \cite{xu2018ontology, cao2019smart}. Xu \emph{et al.} \cite{xu2018ontology} propose an ontology-based fault diagnosis model to integrate, share and reuse of fault diagnosis knowledge for loaders. CBR (case-based reasoning) and RBR (rule-based reasoning) are combined together to achieve effective and accurate fault diagnosis. Cao \emph{et al.} \cite{cao2019smart} present an ontology for representing knowledge of an intelligent condition monitoring systems. The ontology includes manufacturing module, context module, and condition monitoring module, and SWRL \cite{world2004semantic} rules are employed to perform reasoning tasks.

\subsection{Rule-based Approaches}
Rule based approaches are performed based upon the evaluation of on-line monitored data according to a set of rules which is pre-determined by expert knowledge, a.k.a, Expert System (ES). ES stores the so-called domain knowledge extracted by human experts into computers in the form of rules. Usually, rules are expressed in the form: \emph{IF condition, THEN consequence}. The condition portion of a rule is usually a certain type of facts while the consequence can be outcomes that affect the outside world. The process of building ESs involves knowledge acquisition, knowledge representation, and model verification and validation \cite{peng2010current}.

ESs are usually utilized to monitor, interpret, and diagnose systems, and plan PdM activities. Recently, Gul \emph{et al.} \cite{gul2018fuzzy} propose a new risk assessment approach in a rail transportation system by combining Fine–Kinney method and a fuzzy rule-based ES. In \cite{kharlamov2019semantically}, Kharlamov \emph{et al.} design a rule-based language ``SDRL'' for equipment diagnostics in ontology mediated data integration scenarios such as industrial IoT. Its benefits include the ease of formulation and favourable execution time of diagnostic programs with hundreds of pieces of complex equipment. Berredjem \emph{et al.} \cite{berredjem2018bearing} propose a fuzzy expert system to localize bearing faults diagnosis as well as distributed faults. The fuzzy rules are automatically induced from numerical data using an improved range overlaps method. In order to extract diagnosis knowledge or mine rules from database, data mining techniques can be employed in an ES, e.g., ANNs \cite{martinez2015artificial}, decision tree \cite{liu2018fault} and association rule mining \cite{antomarioni2019predictive, grabot2018rule}.
%Compared with model-based approaches, knowledge-based approaches are particularly suitable for large industrial plants since those non-linear real plants are extremely difficult to be modeled and the linear approximation of the model results in large errors. In addition, knowledge-based approaches are able to reduce the complexity when implementing the corresponding safety system and make it flexible, easy to understand and follow. Combining knowledge-based fault diagnosis methods with real-time process variables monitoring will improve the efficiency and reliability of detecting fault behavior and overall effectiveness of the system.


\subsection{Model-based Approaches}
Model-based approaches usually directly tie mathematical models to physical processes. These physical processes have a direct or indirect impact on the health of the relevant systems or components. Model-based approaches for fault diagnosis and prognosis use residuals as features, in which the consistency between the measured results and the expected behavior of the process is checked by the analytical model. Based on this explicit model, residual generation methods such as Kalman filter, system identification and parity relations are used to obtain the residual, which indicates whether there is or will be a fault in the target systems or components.

A variety of models have been examined for fault diagnosis and prognosis, including linear system models \cite{lucifredi2000application}, proportional hazards models \cite{tian2011condition}, exponential models \cite{zhang2018remaining}, Markovian process-based models \cite{sevegnani2017stochastic, aizpurua2018model, cartella2015hidden}, Wiener process based models \cite{li2019wiener, zhang2018degradation} and Gaussian process based models \cite{chen2015condition, pan2016remaining}, etc. These models are employed to solve the maintenance problems in diverse systems and components, e.g., gearboxes \cite{wang2002toward,heyns2012combining}, bearings \cite{hong2012remaining} and rotors \cite{loparo2003model, jalan2009model}, lithium-ion batteries \cite{zhang2018remaining}, aircraft redundant systems \cite{vianna2018predictive}, and building automation systems \cite{tian2011condition, cauchi2017model}. For a complex system, different dependencies \cite{keizer2017condition} (e.g., structural dependence, stochastic dependence and economic dependence) exist among components, thus many approaches also are proposed for multi-component systems \cite{prakash2018model, hu2012opportunistic, hong2014optimal}. In addition, in order to enhance the efficiency of model-baed approaches, machine learning techniques are employed in many studies \cite{luo2010integrated, liang2007model, jung2018combining, slimani2018fusion}.


\subsection{Summary}
Generally, ontology provides a potential way to integrate, share and reuse of context knowledge of a system, but other reasoning methods should be integrated with ontology to achieve PdM. Rule-based approaches can be employed when there is a lot of experience but not enough details to develop accurate quantitative models, e.g.: large industrial plants that are extremely difficult to be modeled and where the linear approximation models may result in large errors. However, a rule-based system often has difficulties in dealing with new faults and acquires complete knowledge to build a reliable rule-base system. Model-based approaches are applicable to where accurate mathematical models can be constructed from physical systems. However, explicit mathematical models may be infeasible for many complex systems. Also, changes in structural dynamics and operating conditions can affect the mathematical model, so it is impossible to model all real-life conditions. Here we list the advantages and limitations of knowledge-based approaches in Table \ref{tbl:knowledge}.

\begin{table*}[]
\begin{center}
\caption{Advantages \& limitations of knowledge-based approaches.}
     \begin{tabular}{ | p{1.5cm} | p{4cm} | p{7cm} | p{2cm}|}
     \hline
      Approaches & Advantages & Limitations & References
       \\ \hline
	  Ontology-based
      & 
      \begin{itemize}
      \item Formally describe the context knowledge
      \item Easy to integrate, share and reuse knowledge%\ldots
      \end{itemize}
      & 
      \begin{itemize}
      \item Lack of reasoning
      \item Acquire complete context knowledge of a system in advance
      \end{itemize}
      &
	  \cite{konys2018ontology, schmidt2017semantic, nunez2018ontoprog, medina2014predictive, voisin2013fleet, xu2018ontology, cao2019smart}
      \\ \hline
      Rule-based
      &
      \begin{itemize}
      \item Reduce the difficulties on exact numeric information
      \item Automate the human intelligence for PdM%\ldots
      \end{itemize}
      &
      \begin{itemize}
      \item Expensive and time-consuming for implementation
      \item Difficult to deal with new faults 
      \item Acquire complete knowledge to build a reliable rule-base system%\ldots
      \end{itemize}
      &
      \cite{gul2018fuzzy, kharlamov2019semantically, berredjem2018bearing, martinez2015artificial, liu2018fault, antomarioni2019predictive, grabot2018rule}
      \\ \hline
      Model-based
      &
      \begin{itemize}
      \item Highly effective and accurate
      \item Models can be reused
      \end{itemize}
      &
      \begin{itemize}
      \item Real-life system is often too stochastic and complex to model
      \item Many mathematics assumptions need to be examined
      \item Various physics parameters need to be determined
      \item Changes in structural dynamics and operating conditions can affect the mathematical model
      \end{itemize}
      &
      \cite{lucifredi2000application, tian2011condition, zhang2018remaining,sevegnani2017stochastic, aizpurua2018model, cartella2015hidden,li2019wiener, zhang2018degradation,chen2015condition, pan2016remaining}, etc.
      \\ \hline
      \end{tabular}
      \label{tbl:knowledge}
\end{center}
\end{table*}



%Most of these physics-based models are unable to be updated with on-line measured data, which limits their effectiveness and flexibility. On the other hand, with significant development of sensors, sensor networks and computing systems, data-driven machine health monitoring models have become more and more attractive. To extract useful knowledge and make appropriate decisions from big data, machine learning techniques have been regarded as a powerful solution. As the hottest subfield of machine learning, deep learning is able to act as a bridge connecting big machinery data and intelligent machine health monitoring.


%With the ever-increasing size of big data produced by modern systems, coupled with the complexities of contextual components for correlating information; can create barriers that were not anticipated by design engineers during the design phase of the system life-cycle. This eventually results in higher levels of uncertainty during the diagnosis process [6]. In this context, novel approaches are required which can configure applications, as well as mechanisms for making better decisions at the system-level. In the nominal environment, such problems warrant advanced capabilities to monitor in-service operations, record and share expert knowledge, and address critical aspects of on-board software. To address this issue, diagnostic systems based on conventional techniques are being replaced by AI-based ones which can increase the efficiency of the monitoring technology.

